Jointly estimating transmissibility and prior immunity from epidemic time series

Infectious disease time series are often used to estimate a pathogen's basic reproduction number, $R_0$. However, fits of epidemic models to time series conflate pathogen transmissibility with pre-existing population immunity, so only the *effective* reproduction number, $R_{eff}$, can be inferred. This composite parameter is the product of the underlying $R_0$ and the pre-epidemic susceptible fraction, $x^-$. We show that a conservation law associated with epidemic momentum---prevalence weighted by potential to infect---makes it possible to disentangle transmissibility from prior immunity and to infer $R_0$ and $x^-$ separately from a single epidemic time series. We test the methodology using stochastic epidemic simulations, and illustrate the approach with a reappraisal of influenza transmissibility during the 1918 pandemic, estimating rather than assuming the degree of prior population immunity. For the autumn wave in Philadelphia, USA, we find $R_0\approx2.7$ and $x^-\approx0.8$, implying that about 20% of the population was already immune before that wave, plausibly as a result of infection during the spring 1918 herald wave.

==> shared/arxiv_external_labels_theory.tex <==
% Generated from the counterpart manuscript auxiliary file.
% It preserves cross-manuscript citation locations without shipping .aux files.
\makeatletter
\newlabel{theory:sec:intro}{{1}{1}{Introduction}{section.1}{}}
\newlabel{theory:sec:intro@cref}{{[section][1][]1}{[1][1][]1}{}{}{}}
\newlabel{theory:eq:SIRstandard}{{1.1}{1}{Introduction}{equation.2}{}}
\newlabel{theory:eq:SIRstandard@cref}{{[equation][1][1]1.1}{[1][1][]1}{}{}{}}
\newlabel{theory:sec:models}{{2}{2}{Epidemic models and phase plane solutions}{section.3}{}}
\newlabel{theory:sec:models@cref}{{[section][2][]2}{[1][2][]2}{}{}{}}
\newlabel{theory:sec:SIR}{{2.1}{2}{SIR model}{subsection.4}{}}
\newlabel{theory:sec:SIR@cref}{{[subsection][1][2]2.1}{[1][2][]2}{}{}{}}
\newlabel{theory:eq:SIR}{{2.1}{2}{SIR model}{equation.5}{}}
\newlabel{theory:eq:SIR@cref}{{[subequation][1][2]2.1}{[1][2][]2}{}{}{}}
\newlabel{theory:eq:SIR;X}{{2.1a}{2}{SIR model}{equation.6}{}}
\newlabel{theory:eq:SIR;X@cref}{{[subequation][1][1]2.1a}{[1][2][]2}{}{}{}}
\newlabel{theory:eq:SIR;Y}{{2.1b}{2}{SIR model}{equation.7}{}}
\newlabel{theory:eq:SIR;Y@cref}{{[subequation][2][1]2.1b}{[1][2][]2}{}{}{}}
\newlabel{theory:eq:initial.simplex.constraint}{{2.2}{2}{SIR model}{equation.8}{}}
\newlabel{theory:eq:initial.simplex.constraint@cref}{{[equation][2][2]2.2}{[1][2][]2}{}{}{}}
\newlabel{theory:fig:phaseplane}{{1}{3}{\textbf {Universality of the susceptible-momentum ($x$-$y$) phase plane.} (\tspanel {A},\tspanel {B}) Time series of the susceptible fraction, $X(\tau )$, and epidemic momentum, $Y(\tau )$, for the SIR and SEIR models [\cref {eq:SIR,eq:SEIR}] with basic reproduction number $\Rn =4$ and initial conditions $(\xinit ,\yinit )=(0.999,0.00075)$. For the SEIR model, the mean latent period is the same as the mean infectious period ($\ell =1$) and the initial exposed and infectious fractions [\cref {eq:SEIR;Eprop,eq:SEIR;Iprop}] are $\epropinit =\ipropinit =\yinit /2$. (\pppanel ) Phase portraits in the susceptible-momentum phase plane, which are identical for both models, and are expressed explicitly by \cref {eq:Yofx}. Trajectories are contours of constant $C(x,y)$ [\protect \cref {eq:FI}] and are labelled with the value of the constant. Both the SIR and SEIR time series on the left correspond to the same (coloured) phase plane trajectory on the right. The dotted line is the biological boundary, $x+y=1$. The dashed line indicates peak epidemic momentum, which occurs at $x=\xpeak =\frac {1}{\Rn }$. The points plotted on the $x$-axis are at $\xm $ (white) and $\xp $ (black), the pre- and post-epidemic susceptible proportions for each trajectory [\cref {eq:xpm}]}{figure.12}{}}
\newlabel{theory:fig:phaseplane@cref}{{[figure][1][]1}{[1][3][]3}{}{}{}}
\newlabel{theory:sec:ppsol}{{2.2}{3}{Phase plane solution}{subsection.9}{}}
\newlabel{theory:sec:ppsol@cref}{{[subsection][2][2]2.2}{[1][2][]3}{}{}{}}
\newlabel{theory:eq:dYdx}{{2.3}{3}{Phase plane solution}{equation.10}{}}
\newlabel{theory:eq:dYdx@cref}{{[equation][3][2]2.3}{[1][2][]3}{}{}{}}
\newlabel{theory:eq:Yofx}{{2.4}{3}{Phase plane solution}{equation.11}{}}
\newlabel{theory:eq:Yofx@cref}{{[equation][4][2]2.4}{[1][2][]3}{}{}{}}
\newlabel{theory:sec:SEIR}{{2.3}{3}{SEIR model}{subsection.14}{}}
\newlabel{theory:sec:SEIR@cref}{{[subsection][3][2]2.3}{[1][3][]3}{}{}{}}
\newlabel{theory:eq:SEIR}{{2.5}{4}{SEIR model}{equation.15}{}}
\newlabel{theory:eq:SEIR@cref}{{[subequation][5][2]2.5}{[1][3][]4}{}{}{}}
\newlabel{theory:eq:SEIR;X}{{2.5a}{4}{SEIR model}{equation.16}{}}
\newlabel{theory:eq:SEIR;X@cref}{{[subequation][1][5]2.5a}{[1][3][]4}{}{}{}}
\newlabel{theory:eq:SEIR;Eprop}{{2.5b}{4}{SEIR model}{equation.17}{}}
\newlabel{theory:eq:SEIR;Eprop@cref}{{[subequation][2][5]2.5b}{[1][3][]4}{}{}{}}
\newlabel{theory:eq:SEIR;Iprop}{{2.5c}{4}{SEIR model}{equation.18}{}}
\newlabel{theory:eq:SEIR;Iprop@cref}{{[subequation][3][5]2.5c}{[1][3][]4}{}{}{}}
\newlabel{theory:eq:XYF}{{2.6}{4}{SEIR model}{equation.19}{}}
\newlabel{theory:eq:XYF@cref}{{[subequation][6][2]2.6}{[1][4][]4}{}{}{}}
\newlabel{theory:eq:XYF;X}{{2.6a}{4}{SEIR model}{equation.20}{}}
\newlabel{theory:eq:XYF;X@cref}{{[subequation][1][6]2.6a}{[1][4][]4}{}{}{}}
\newlabel{theory:eq:XYF;Y}{{2.6b}{4}{SEIR model}{equation.21}{}}
\newlabel{theory:eq:XYF;Y@cref}{{[subequation][2][6]2.6b}{[1][4][]4}{}{}{}}
\newlabel{theory:sec:SI1I2R}{{2.4}{4}{SI$_1$I$_2$R model}{subsection.22}{}}
\newlabel{theory:sec:SI1I2R@cref}{{[subsection][4][2]2.4}{[1][4][]4}{}{}{}}
\newlabel{theory:eq:SI1I2R}{{2.7}{4}{SI$_1$I$_2$R model}{equation.23}{}}
\newlabel{theory:eq:SI1I2R@cref}{{[subequation][7][2]2.7}{[1][4][]4}{}{}{}}
\newlabel{theory:eq:SI1I2R;X}{{2.7a}{4}{SI$_1$I$_2$R model}{equation.24}{}}
\newlabel{theory:eq:SI1I2R;X@cref}{{[subequation][1][7]2.7a}{[1][4][]4}{}{}{}}
\newlabel{theory:eq:SI1I2R;Y1}{{2.7b}{4}{SI$_1$I$_2$R model}{equation.25}{}}
\newlabel{theory:eq:SI1I2R;Y1@cref}{{[subequation][2][7]2.7b}{[1][4][]4}{}{}{}}
\newlabel{theory:eq:SI1I2R;Y2}{{2.7c}{4}{SI$_1$I$_2$R model}{equation.26}{}}
\newlabel{theory:eq:SI1I2R;Y2@cref}{{[subequation][3][7]2.7c}{[1][4][]4}{}{}{}}
\newlabel{theory:eq:SI1I2R;prev}{{2.8}{4}{SI$_1$I$_2$R model}{equation.27}{}}
\newlabel{theory:eq:SI1I2R;prev@cref}{{[equation][8][2]2.8}{[1][4][]4}{}{}{}}
\newlabel{theory:eq:SI1I2R;prevdot}{{2.9}{4}{SI$_1$I$_2$R model}{equation.28}{}}
\newlabel{theory:eq:SI1I2R;prevdot@cref}{{[equation][9][2]2.9}{[1][4][]4}{}{}{}}
\newlabel{theory:eq:SI1I2R;prevalence.phase}{{2.10}{4}{SI$_1$I$_2$R model}{equation.29}{}}
\newlabel{theory:eq:SI1I2R;prevalence.phase@cref}{{[equation][10][2]2.10}{[1][4][]4}{}{}{}}
\newlabel{theory:sec:re}{{2.5}{5}{Renewal equation}{subsection.30}{}}
\newlabel{theory:sec:re@cref}{{[subsection][5][2]2.5}{[1][5][]5}{}{}{}}
\newlabel{theory:eq:re}{{2.11}{5}{Renewal equation}{equation.32}{}}
\newlabel{theory:eq:re@cref}{{[subequation][11][2]2.11}{[1][5][]5}{}{}{}}
\newlabel{theory:eq:re;X}{{2.11a}{5}{Renewal equation}{equation.33}{}}
\newlabel{theory:eq:re;X@cref}{{[subequation][1][11]2.11a}{[1][5][]5}{}{}{}}
\newlabel{theory:eq:re;FoI}{{2.11b}{5}{Renewal equation}{equation.34}{}}
\newlabel{theory:eq:re;FoI@cref}{{[subequation][2][11]2.11b}{[1][5][]5}{}{}{}}
\newlabel{theory:eq:re;inc}{{2.12}{5}{Renewal equation}{equation.35}{}}
\newlabel{theory:eq:re;inc@cref}{{[equation][12][2]2.12}{[1][5][]5}{}{}{}}
\newlabel{theory:eq:re.initial.history}{{2.13}{6}{Renewal equation}{equation.36}{}}
\newlabel{theory:eq:re.initial.history@cref}{{[equation][13][2]2.13}{[1][5][]6}{}{}{}}
\newlabel{theory:eq:re.initial.FoI}{{2.14}{6}{Renewal equation}{equation.37}{}}
\newlabel{theory:eq:re.initial.FoI@cref}{{[equation][14][2]2.14}{[1][6][]6}{}{}{}}
\newlabel{theory:sec:epimom.etc}{{3}{6}{Epidemic momentum}{section.38}{}}
\newlabel{theory:sec:epimom.etc@cref}{{[section][3][]3}{[1][6][]6}{}{}{}}
\newlabel{theory:sec:epimom}{{3.1}{6}{Definition of epidemic momentum}{subsection.39}{}}
\newlabel{theory:sec:epimom@cref}{{[subsection][1][3]3.1}{[1][6][]6}{}{}{}}
\newlabel{theory:eq:GI.survival}{{3.1}{6}{Definition of epidemic momentum}{equation.40}{}}
\newlabel{theory:eq:GI.survival@cref}{{[equation][1][3]3.1}{[1][6][]6}{}{}{}}
\newlabel{theory:eq:Ra}{{3.2}{6}{Definition of epidemic momentum}{equation.41}{}}
\newlabel{theory:eq:Ra@cref}{{[equation][2][3]3.2}{[1][6][]6}{}{}{}}
\newlabel{theory:eq:re.Y}{{3.3}{6}{Definition of epidemic momentum}{equation.43}{}}
\newlabel{theory:eq:re.Y@cref}{{[equation][3][3]3.3}{[1][6][]6}{}{}{}}
\newlabel{theory:eq:re.Y.history}{{3.4}{7}{Definition of epidemic momentum}{equation.44}{}}
\newlabel{theory:eq:re.Y.history@cref}{{[equation][4][3]3.4}{[1][7][]7}{}{}{}}
\newlabel{theory:eq:re.Ydot}{{3.5}{7}{Definition of epidemic momentum}{equation.45}{}}
\newlabel{theory:eq:re.Ydot@cref}{{[equation][5][3]3.5}{[1][7][]7}{}{}{}}
\newlabel{theory:eq:re;yinit}{{3.6}{7}{Definition of epidemic momentum}{equation.46}{}}
\newlabel{theory:eq:re;yinit@cref}{{[equation][6][3]3.6}{[1][7][]7}{}{}{}}
\newlabel{theory:sec:phaseplane}{{3.2}{8}{Universality of the SIR phase portrait}{subsection.47}{}}
\newlabel{theory:sec:phaseplane@cref}{{[subsection][2][3]3.2}{[1][7][]8}{}{}{}}
\newlabel{theory:sec:timechange}{{3.3}{8}{Equivalence of generic and SIR epidemics via time transformation}{subsection.48}{}}
\newlabel{theory:sec:timechange@cref}{{[subsection][3][3]3.3}{[1][8][]8}{}{}{}}
\newlabel{theory:eq:timechange}{{3.7}{8}{Equivalence of generic and SIR epidemics via time transformation}{equation.49}{}}
\newlabel{theory:eq:timechange@cref}{{[equation][7][3]3.7}{[1][8][]8}{}{}{}}
\newlabel{theory:sec:FI}{{3.4}{8}{A first integral for generic epidemics}{subsection.50}{}}
\newlabel{theory:sec:FI@cref}{{[subsection][4][3]3.4}{[1][8][]8}{}{}{}}
\newlabel{theory:eq:FI.derivation}{{3.8}{8}{A first integral for generic epidemics}{equation.51}{}}
\newlabel{theory:eq:FI.derivation@cref}{{[equation][8][3]3.8}{[1][8][]8}{}{}{}}
\newlabel{theory:eq:FI}{{3.9}{8}{A first integral for generic epidemics}{equation.52}{}}
\newlabel{theory:eq:FI@cref}{{[equation][9][3]3.9}{[1][8][]8}{}{}{}}
\newlabel{theory:eq:Volterra}{{3.10}{8}{A first integral for generic epidemics}{equation.53}{}}
\newlabel{theory:eq:Volterra@cref}{{[equation][10][3]3.10}{[1][8][]8}{}{}{}}
\newlabel{theory:eq:FI.value}{{3.11}{8}{A first integral for generic epidemics}{equation.54}{}}
\newlabel{theory:eq:FI.value@cref}{{[equation][11][3]3.11}{[1][8][]8}{}{}{}}
\newlabel{theory:sec:pp.pi.fs}{{3.5}{9}{Prior immunity and final size from the universal phase portrait}{subsection.55}{}}
\newlabel{theory:sec:pp.pi.fs@cref}{{[subsection][5][3]3.5}{[1][8][]9}{}{}{}}
\newlabel{theory:sec:explicit.xpm}{{3.5.1}{9}{Explicit expressions}{subsubsection.56}{}}
\newlabel{theory:sec:explicit.xpm@cref}{{[subsubsection][1][3,5]3.5.1}{[1][8][]9}{}{}{}}
\newlabel{theory:eq:Xofy}{{3.12}{9}{Explicit expressions}{equation.57}{}}
\newlabel{theory:eq:Xofy@cref}{{[subequation][12][3]3.12}{[1][8][]9}{}{}{}}
\newlabel{theory:eq:Xpmofy}{{3.12b}{9}{Explicit expressions}{equation.59}{}}
\newlabel{theory:eq:Xpmofy@cref}{{[subequation][2][12]3.12b}{[1][9][]9}{}{}{}}
\newlabel{theory:eq:xpm}{{3.13}{9}{Explicit expressions}{equation.60}{}}
\newlabel{theory:eq:xpm@cref}{{[equation][13][3]3.13}{[1][9][]9}{}{}{}}
\newlabel{theory:eq:zm}{{3.14}{9}{Explicit expressions}{equation.61}{}}
\newlabel{theory:eq:zm@cref}{{[equation][14][3]3.14}{[1][9][]9}{}{}{}}
\newlabel{theory:eq:zp}{{3.15}{9}{Explicit expressions}{equation.62}{}}
\newlabel{theory:eq:zp@cref}{{[equation][15][3]3.15}{[1][9][]9}{}{}{}}
\newlabel{theory:sec:naive.final.size}{{3.5.2}{9}{Relationship to na\"ive final size}{subsubsection.63}{}}
\newlabel{theory:sec:naive.final.size@cref}{{[subsubsection][2][3,5]3.5.2}{[1][9][]9}{}{}{}}
\newlabel{theory:eq:R.vs.Reff.identity}{{3.16}{9}{Relationship to na\"ive final size}{equation.64}{}}
\newlabel{theory:eq:R.vs.Reff.identity@cref}{{[equation][16][3]3.16}{[1][9][]9}{}{}{}}
\newlabel{theory:eq:zp.vs.naive}{{3.17}{9}{Relationship to na\"ive final size}{equation.65}{}}
\newlabel{theory:eq:zp.vs.naive@cref}{{[equation][17][3]3.17}{[1][9][]9}{}{}{}}
\newlabel{theory:sec:constraints.final.size}{{3.5.3}{10}{Constraints on initial conditions and final size}{subsubsection.66}{}}
\newlabel{theory:sec:constraints.final.size@cref}{{[subsubsection][3][3,5]3.5.3}{[1][9][]10}{}{}{}}
\newlabel{theory:eq:yinit.constraint}{{3.18}{10}{Constraints on initial conditions and final size}{equation.67}{}}
\newlabel{theory:eq:yinit.constraint@cref}{{[equation][18][3]3.18}{[1][10][]10}{}{}{}}
\newlabel{theory:eq:xp.lt.xm}{{3.19}{10}{Constraints on initial conditions and final size}{equation.68}{}}
\newlabel{theory:eq:xp.lt.xm@cref}{{[equation][19][3]3.19}{[1][10][]10}{}{}{}}
\newlabel{theory:sec:constraint.Rn}{{3.5.4}{10}{Constraint on $\Rn $ from given initial conditions}{subsubsection.69}{}}
\newlabel{theory:sec:constraint.Rn@cref}{{[subsubsection][4][3,5]3.5.4}{[1][10][]10}{}{}{}}
\newlabel{theory:eq:Rnmin}{{3.20}{10}{Constraint on $\Rn $ from given initial conditions}{equation.70}{}}
\newlabel{theory:eq:Rnmin@cref}{{[equation][20][3]3.20}{[1][10][]10}{}{}{}}
\newlabel{theory:sec:non-monotonicity.final.size}{{3.5.5}{10}{Non-monotonicity of final size}{subsubsection.71}{}}
\newlabel{theory:sec:non-monotonicity.final.size@cref}{{[subsubsection][5][3,5]3.5.5}{[1][10][]10}{}{}{}}
\newlabel{theory:eq:zpmin.Rnstar.leading.approx}{{3.21}{10}{Non-monotonicity of final size}{equation.72}{}}
\newlabel{theory:eq:zpmin.Rnstar.leading.approx@cref}{{[equation][21][3]3.21}{[1][10][]10}{}{}{}}
\newlabel{theory:eq:zp.before.after.tauinit}{{3.22}{10}{Non-monotonicity of final size}{equation.73}{}}
\newlabel{theory:eq:zp.before.after.tauinit@cref}{{[equation][22][3]3.22}{[1][10][]10}{}{}{}}
\newlabel{theory:tab:zp.critical.values}{{1}{11}{Critical points and limiting values of $\zp (\Rn )$ for the initial conditions used in \cref {fig:zpm}. The lower bound $\Rnmin $ is the value at which $\xm =1$. The quantities $\Rnstarmin $ and $\Rnstarmax $ denote the local minimum and local maximum points of $\zp (\Rn )$, respectively. The limiting value is $\zplim =\xinit +\yinit =\lim _{\Rn \to \infty }\zp (\Rn )$. The dagger marks the case in which the local minimum lies below $\Rnmin $, so it would imply $\xm >1$}{table.76}{}}
\newlabel{theory:tab:zp.critical.values@cref}{{[table][1][]1}{[1][11][]11}{}{}{}}
\newlabel{theory:fig:zpm}{{2}{12}{\textbf {Prior immunity $(\zm )$ {\upshape [\cref {eq:zm}]}, total post-epidemic immune fraction $(\zptot =1-\xp )$ and final size $(\zp )$ {\upshape [\cref {eq:zp}]} vs $\Rn $ for six given initial states.} The vertical dotted grey line is at $\Rn ={1}/({\xinit -\yinit })$, which closely approximates the reproduction number at which the final size is minimized {\upshape [\cref {eq:zpmin.Rnstar.leading.approx}]}. Non-monotonicity of the final size is possible because the initial conditions are fixed as $\Rn $ is increased (see \cref {sec:non-monotonicity.final.size}). For $(\xinit ,\yinit )=(0.9,0.01)$ (bottom left panel), the exact critical-point condition for $\zp (\Rn )$ has two solutions, $\Rnstar \approx 1.124$ and $\Rnstar \approx 9.38$. The leading approximation \labelcref {eq:zpmin.Rnstar.leading.approx}, indicated in the figure, agrees with the exact lower critical point to four significant digits. However, this point lies below $\Rnmin \approx 1.171$ {\upshape [\cref {eq:Rnmin}]}, so it would imply a pre-epidemic susceptible fraction greater than one. The second critical point is a large-$\Rn $ local maximum, beyond which $\zp (\Rn )$ decreases to $\xinit +\yinit =0.91$. See \cref {tab:zp.critical.values}}{figure.74}{}}
\newlabel{theory:fig:zpm@cref}{{[figure][2][]2}{[1][11][]12}{}{}{}}
\newlabel{theory:sec:rise.fall}{{3.6}{13}{Rising and falling tail exponents, $\lampm $}{subsection.78}{}}
\newlabel{theory:sec:rise.fall@cref}{{[subsection][6][3]3.6}{[1][13][]13}{}{}{}}
\newlabel{theory:eq:lamLaplace}{{3.23}{13}{Rising and falling tail exponents, $\lampm $}{equation.79}{}}
\newlabel{theory:eq:lamLaplace@cref}{{[subequation][23][3]3.23}{[1][13][]13}{}{}{}}
\newlabel{theory:eq:lamLaplace;lam}{{3.23a}{13}{Rising and falling tail exponents, $\lampm $}{equation.80}{}}
\newlabel{theory:eq:lamLaplace;lam@cref}{{[subequation][1][23]3.23a}{[1][13][]13}{}{}{}}
\newlabel{theory:eq:lamLaplace;Laplace}{{3.23b}{13}{Rising and falling tail exponents, $\lampm $}{equation.81}{}}
\newlabel{theory:eq:lamLaplace;Laplace@cref}{{[subequation][2][23]3.23b}{[1][13][]13}{}{}{}}
\newlabel{theory:sec:est.Rn.xm}{{3.7}{13}{Momentum, endpoints, and tail exponents}{subsection.84}{}}
\newlabel{theory:sec:est.Rn.xm@cref}{{[subsection][7][3]3.7}{[1][13][]13}{}{}{}}
\newlabel{theory:eq:R.C.lampm}{{3.24}{13}{Momentum, endpoints, and tail exponents}{equation.85}{}}
\newlabel{theory:eq:R.C.lampm@cref}{{[equation][24][3]3.24}{[1][13][]13}{}{}{}}
\newlabel{theory:eq:compute}{{3.25}{13}{Momentum, endpoints, and tail exponents}{equation.86}{}}
\newlabel{theory:eq:compute@cref}{{[subequation][25][3]3.25}{[1][13][]13}{}{}{}}
\newlabel{theory:eq:zm.compute}{{3.25a}{13}{Momentum, endpoints, and tail exponents}{equation.87}{}}
\newlabel{theory:eq:zm.compute@cref}{{[subequation][1][25]3.25a}{[1][13][]13}{}{}{}}
\newlabel{theory:eq:zp.compute}{{3.25b}{13}{Momentum, endpoints, and tail exponents}{equation.88}{}}
\newlabel{theory:eq:zp.compute@cref}{{[subequation][2][25]3.25b}{[1][13][]13}{}{}{}}
\newlabel{theory:tab:GI.properties}{{2}{14}{Intrinsic generation-interval distributions, Laplace transforms, and tail exponents for the SIR model \labelcref {eq:SIR}, SEIR model \labelcref {eq:SEIR}, and the \RE \cref {eq:re} with a Gamma distributed intrinsic generation interval $g(\aoi )$ ($\aoi $ denotes age of infection). In the SEIR row, $\ell $ is the ratio of the mean latent period to the mean infectious period. In the Gamma GI row, $a>0$ and $b>0$ are the Gamma shape and rate parameters, respectively, so the mean is $a/b$ and the variance is $a/b^2$}{table.82}{}}
\newlabel{theory:tab:GI.properties@cref}{{[table][2][]2}{[1][13][]14}{}{}{}}
\newlabel{theory:eq:V=V}{{3.26}{14}{Momentum, endpoints, and tail exponents}{equation.89}{}}
\newlabel{theory:eq:V=V@cref}{{[equation][26][3]3.26}{[1][13][]14}{}{}{}}
\newlabel{theory:sec:Discussion}{{4}{14}{Discussion}{section.90}{}}
\newlabel{theory:sec:Discussion@cref}{{[section][4][]4}{[1][14][]14}{}{}{}}
\newlabel{theory:sec:physics.analogies}{{4.1}{15}{Physics analogies}{subsection.91}{}}
\newlabel{theory:sec:physics.analogies@cref}{{[subsection][1][4]4.1}{[1][15][]15}{}{}{}}
\newlabel{theory:eq:dY.again}{{4.1}{15}{Physics analogies}{equation.92}{}}
\newlabel{theory:eq:dY.again@cref}{{[equation][1][4]4.1}{[1][15][]15}{}{}{}}
\newlabel{theory:eq:epidemic.charge}{{4.2}{15}{Physics analogies}{equation.93}{}}
\newlabel{theory:eq:epidemic.charge@cref}{{[equation][2][4]4.2}{[1][15][]15}{}{}{}}
\newlabel{theory:sec:ext.gen}{{4.2}{16}{Extensions and Generalizations}{subsection.94}{}}
\newlabel{theory:sec:ext.gen@cref}{{[subsection][2][4]4.2}{[1][16][]16}{}{}{}}
\newlabel{theory:sec:nli}{{4.2.1}{16}{Nonlinear incidence}{subsubsection.95}{}}
\newlabel{theory:sec:nli@cref}{{[subsubsection][1][4,2]4.2.1}{[1][16][]16}{}{}{}}
\newlabel{theory:sec:approx}{{4.2.2}{16}{Approximation of solutions of epidemic models}{subsubsection.96}{}}
\newlabel{theory:sec:approx@cref}{{[subsubsection][2][4,2]4.2.2}{[1][16][]16}{}{}{}}
\newlabel{theory:sec:time.dep}{{4.2.3}{16}{Time-dependent transmission rates}{subsubsection.97}{}}
\newlabel{theory:sec:time.dep@cref}{{[subsubsection][3][4,2]4.2.3}{[1][16][]16}{}{}{}}
\newlabel{theory:sec:srpb}{{4.2.4}{16}{Susceptible recruitment}{subsubsection.98}{}}
\newlabel{theory:sec:srpb@cref}{{[subsubsection][4][4,2]4.2.4}{[1][16][]16}{}{}{}}
\newlabel{theory:sec:pop.mom}{{4.2.5}{17}{Population momentum more generally}{subsubsection.99}{}}
\newlabel{theory:sec:pop.mom@cref}{{[subsubsection][5][4,2]4.2.5}{[1][17][]17}{}{}{}}
\newlabel{theory:sec:conclusion}{{4.3}{17}{Conclusion}{subsection.100}{}}
\newlabel{theory:sec:conclusion@cref}{{[subsection][3][4]4.3}{[1][17][]17}{}{}{}}
\newlabel{theory:app:re.to.seir}{{A}{17}{Equivalence of the \RE and compartmental models}{appendix.101}{}}
\newlabel{theory:app:re.to.seir@cref}{{[appendix][1][2147483647]A}{[1][17][]17}{}{}{}}
\newlabel{theory:eq:re.SEIR;X}{{A.1a}{17}{Equivalence of the \RE and compartmental models}{equation.103}{}}
\newlabel{theory:eq:re.SEIR;X@cref}{{[subequation][1][2147483647,1]A.1a}{[1][17][]17}{}{}{}}
\newlabel{theory:eq:re.SEIR;Iprop}{{A.1b}{17}{Equivalence of the \RE and compartmental models}{equation.104}{}}
\newlabel{theory:eq:re.SEIR;Iprop@cref}{{[subequation][2][2147483647,1]A.1b}{[1][17][]17}{}{}{}}
\newlabel{theory:eq:ddtauIprop}{{A.2a}{17}{Equivalence of the \RE and compartmental models}{equation.106}{}}
\newlabel{theory:eq:ddtauIprop@cref}{{[subequation][1][2147483647,2]A.2a}{[1][17][]17}{}{}{}}
\newlabel{theory:eq:SEIR-E}{{A.7}{18}{Equivalence of the \RE and compartmental models}{equation.113}{}}
\newlabel{theory:eq:SEIR-E@cref}{{[equation][7][2147483647,1]A.7}{[1][18][]18}{}{}{}}
\newlabel{theory:app:y.equiv}{{B}{18}{\texorpdfstring {Equivalence of integral and ODE representations of epidemic momentum $Y(\tau )$}{Equivalent representations of epidemic momentum Y(tau)}}{appendix.119}{}}
\newlabel{theory:app:y.equiv@cref}{{[appendix][2][2147483647]B}{[1][18][]18}{}{}{}}
\newlabel{theory:subapp:re.to.Y}{{B.1}{18}{The \RE and the ODE for $Y$ imply the integral form of $Y$}{subsection.120}{}}
\newlabel{theory:subapp:re.to.Y@cref}{{[subappendix][1][2147483647,2]B.1}{[1][18][]18}{}{}{}}
\newlabel{theory:eq:Y.ode.inc}{{B.1}{18}{The \RE and the ODE for $Y$ imply the integral form of $Y$}{equation.121}{}}
\newlabel{theory:eq:Y.ode.inc@cref}{{[equation][1][2147483647,2]B.1}{[1][18][]18}{}{}{}}
\newlabel{theory:eq:Y.int.inc}{{B.2}{19}{The \RE and the ODE for $Y$ imply the integral form of $Y$}{equation.122}{}}
\newlabel{theory:eq:Y.int.inc@cref}{{[subequation][2][2147483647,2]B.2}{[1][18][]19}{}{}{}}
\newlabel{theory:eq:integral-diff}{{B.2d}{19}{The \RE and the ODE for $Y$ imply the integral form of $Y$}{equation.126}{}}
\newlabel{theory:eq:integral-diff@cref}{{[subequation][4][2147483647,2]B.2d}{[1][18][]19}{}{}{}}
\newlabel{theory:eq:inner-rewritten}{{B.3}{19}{The \RE and the ODE for $Y$ imply the integral form of $Y$}{equation.127}{}}
\newlabel{theory:eq:inner-rewritten@cref}{{[equation][3][2147483647,2]B.3}{[1][19][]19}{}{}{}}
\newlabel{theory:eq:double-integral-before-switch}{{B.4}{19}{The \RE and the ODE for $Y$ imply the integral form of $Y$}{equation.128}{}}
\newlabel{theory:eq:double-integral-before-switch@cref}{{[equation][4][2147483647,2]B.4}{[1][19][]19}{}{}{}}
\newlabel{theory:eq:first-final}{{B.5}{19}{The \RE and the ODE for $Y$ imply the integral form of $Y$}{equation.129}{}}
\newlabel{theory:eq:first-final@cref}{{[equation][5][2147483647,2]B.5}{[1][19][]19}{}{}{}}
\newlabel{theory:eq:Y.int.inc;d}{{B.6}{19}{The \RE and the ODE for $Y$ imply the integral form of $Y$}{equation.131}{}}
\newlabel{theory:eq:Y.int.inc;d@cref}{{[equation][6][2147483647,2]B.6}{[1][19][]19}{}{}{}}
\newlabel{theory:subapp:Y.to.re}{{B.2}{19}{The integral form and ODE for $Y$ together imply the \RE }{subsection.132}{}}
\newlabel{theory:subapp:Y.to.re@cref}{{[subappendix][2][2147483647,2]B.2}{[1][19][]19}{}{}{}}
\newlabel{theory:eq:FoI.via.int.by.parts}{{B.7}{20}{The integral form and ODE for $Y$ together imply the \RE }{equation.133}{}}
\newlabel{theory:eq:FoI.via.int.by.parts@cref}{{[equation][7][2147483647,2]B.7}{[1][19][]20}{}{}{}}
\newlabel{theory:app:lampm.re}{{C}{20}{\texorpdfstring {Asymptotic growth rates $\lampm $ from the renewal equation}{Asymptotic growth rates lambda+/- from the renewal equation}}{appendix.135}{}}
\newlabel{theory:app:lampm.re@cref}{{[appendix][3][2147483647]C}{[1][20][]20}{}{}{}}
\newlabel{theory:subapp:lampm.re.sir}{{C.1}{20}{$\lampm $ for the SIR model}{subsection.136}{}}
\newlabel{theory:subapp:lampm.re.sir@cref}{{[subappendix][1][2147483647,3]C.1}{[1][20][]20}{}{}{}}
\newlabel{theory:subapp:lampm.re.generic}{{C.2}{20}{$\lampm $ from the \RE }{subsection.140}{}}
\newlabel{theory:subapp:lampm.re.generic@cref}{{[subappendix][2][2147483647,3]C.2}{[1][20][]20}{}{}{}}
\newlabel{theory:eq:inc;tail}{{C.4}{20}{$\lampm $ from the \RE }{equation.141}{}}
\newlabel{theory:eq:inc;tail@cref}{{[equation][4][2147483647,3]C.4}{[1][20][]20}{}{}{}}
\newlabel{theory:eq:rLaplace}{{C.6}{20}{$\lampm $ from the \RE }{equation.143}{}}
\newlabel{theory:eq:rLaplace@cref}{{[equation][6][2147483647,3]C.6}{[1][20][]20}{}{}{}}
\newlabel{theory:eq:Yinc}{{C.8}{21}{$\lampm $ from the \RE }{equation.145}{}}
\newlabel{theory:eq:Yinc@cref}{{[equation][8][2147483647,3]C.8}{[1][20][]21}{}{}{}}
\newlabel{theory:eq:Yinc.const}{{C.9}{21}{$\lampm $ from the \RE }{equation.146}{}}
\newlabel{theory:eq:Yinc.const@cref}{{[equation][9][2147483647,3]C.9}{[1][20][]21}{}{}{}}
\newlabel{theory:app:lampm.re.exist}{{C.3}{21}{Existence of the tail exponents}{subsection.147}{}}
\newlabel{theory:app:lampm.re.exist@cref}{{[subappendix][3][2147483647,3]C.3}{[1][21][]21}{}{}{}}
\newlabel{theory:eq:bounded.support.Laplace}{{C.10}{21}{Existence of the tail exponents}{equation.148}{}}
\newlabel{theory:eq:bounded.support.Laplace@cref}{{[equation][10][2147483647,3]C.10}{[1][21][]21}{}{}{}}
\newlabel{theory:eq:r.ineq}{{C.11}{21}{Existence of the tail exponents}{equation.149}{}}
\newlabel{theory:eq:r.ineq@cref}{{[equation][11][2147483647,3]C.11}{[1][21][]21}{}{}{}}
\newlabel{theory:eq:lognormal.g}{{C.12}{22}{Existence of the tail exponents}{equation.150}{}}
\newlabel{theory:eq:lognormal.g@cref}{{[equation][12][2147483647,3]C.12}{[1][22][]22}{}{}{}}
\newlabel{theory:eq:lognormal.mgf}{{C.13}{22}{Existence of the tail exponents}{equation.151}{}}
\newlabel{theory:eq:lognormal.mgf@cref}{{[equation][13][2147483647,3]C.13}{[1][22][]22}{}{}{}}
\newlabel{theory:app:tail.exponents}{{C.4}{22}{Tail exponents for specific models}{subsection.152}{}}
\newlabel{theory:app:tail.exponents@cref}{{[subappendix][4][2147483647,3]C.4}{[1][22][]22}{}{}{}}
\newlabel{theory:app:yinit.from.incinit}{{D}{22}{Initial epidemic momentum $\yinit $ from initial incidence $\incinit $}{appendix.153}{}}
\newlabel{theory:app:yinit.from.incinit@cref}{{[appendix][4][2147483647]D}{[1][22][]22}{}{}{}}
\newlabel{theory:eq:inc.init}{{D.1}{22}{Initial epidemic momentum $\yinit $ from initial incidence $\incinit $}{equation.154}{}}
\newlabel{theory:eq:inc.init@cref}{{[equation][1][2147483647,4]D.1}{[1][22][]22}{}{}{}}
\newlabel{theory:Yinc.init}{{D.2}{22}{Initial epidemic momentum $\yinit $ from initial incidence $\incinit $}{equation.155}{}}
\newlabel{theory:Yinc.init@cref}{{[equation][2][2147483647,4]D.2}{[1][22][]22}{}{}{}}
\newlabel{theory:app:momentum.peak}{{E}{22}{Existence of the momentum peak}{appendix.156}{}}
\newlabel{theory:app:momentum.peak@cref}{{[appendix][5][2147483647]E}{[1][22][]22}{}{}{}}
\newlabel{theory:eq:Y.asymptotic.split}{{E.1}{23}{Existence of the momentum peak}{equation.157}{}}
\newlabel{theory:eq:Y.asymptotic.split@cref}{{[subequation][1][2147483647,5]E.1}{[1][22][]23}{}{}{}}
\newlabel{theory:eq:Y.asymptotic.split;sum}{{E.1a}{23}{Existence of the momentum peak}{equation.158}{}}
\newlabel{theory:eq:Y.asymptotic.split;sum@cref}{{[subequation][1][2147483647,1]E.1a}{[1][22][]23}{}{}{}}
\newlabel{theory:eq:Y.asymptotic.split;hist}{{E.1b}{23}{Existence of the momentum peak}{equation.159}{}}
\newlabel{theory:eq:Y.asymptotic.split;hist@cref}{{[subequation][2][2147483647,1]E.1b}{[1][22][]23}{}{}{}}
\newlabel{theory:eq:Y.asymptotic.split;new}{{E.1c}{23}{Existence of the momentum peak}{equation.160}{}}
\newlabel{theory:eq:Y.asymptotic.split;new@cref}{{[subequation][3][2147483647,1]E.1c}{[1][22][]23}{}{}{}}
\newlabel{theory:eq:Y.asymptotic.hist.bound}{{E.2}{23}{Existence of the momentum peak}{equation.161}{}}
\newlabel{theory:eq:Y.asymptotic.hist.bound@cref}{{[equation][2][2147483647,5]E.2}{[1][23][]23}{}{}{}}
\newlabel{theory:eq:Y.asymptotic.hist.limit}{{E.3}{23}{Existence of the momentum peak}{equation.162}{}}
\newlabel{theory:eq:Y.asymptotic.hist.limit@cref}{{[equation][3][2147483647,5]E.3}{[1][23][]23}{}{}{}}
\newlabel{theory:eq:post.initial.total.incidence}{{E.4}{23}{Existence of the momentum peak}{equation.163}{}}
\newlabel{theory:eq:post.initial.total.incidence@cref}{{[equation][4][2147483647,5]E.4}{[1][23][]23}{}{}{}}
\newlabel{theory:eq:Y.asymptotic.new.bound}{{E.5}{23}{Existence of the momentum peak}{equation.164}{}}
\newlabel{theory:eq:Y.asymptotic.new.bound@cref}{{[equation][5][2147483647,5]E.5}{[1][23][]23}{}{}{}}
\newlabel{theory:eq:Y.asymptotic.limit}{{E.6}{23}{Existence of the momentum peak}{equation.165}{}}
\newlabel{theory:eq:Y.asymptotic.limit@cref}{{[equation][6][2147483647,5]E.6}{[1][23][]23}{}{}{}}
\newlabel{theory:eq:history.future.FoI}{{E.7}{24}{Existence of the momentum peak}{equation.166}{}}
\newlabel{theory:eq:history.future.FoI@cref}{{[equation][7][2147483647,5]E.7}{[1][23][]24}{}{}{}}
\newlabel{theory:eq:history.future.FoI.total}{{E.8}{24}{Existence of the momentum peak}{equation.167}{}}
\newlabel{theory:eq:history.future.FoI.total@cref}{{[subequation][8][2147483647,5]E.8}{[1][23][]24}{}{}{}}
\newlabel{theory:eq:history.future.FoI.total;original}{{E.8a}{24}{Existence of the momentum peak}{equation.168}{}}
\newlabel{theory:eq:history.future.FoI.total;original@cref}{{[subequation][1][2147483647,8]E.8a}{[1][24][]24}{}{}{}}
\newlabel{theory:eq:history.future.FoI.total;reordered}{{E.8b}{24}{Existence of the momentum peak}{equation.169}{}}
\newlabel{theory:eq:history.future.FoI.total;reordered@cref}{{[subequation][2][2147483647,8]E.8b}{[1][24][]24}{}{}{}}
\newlabel{theory:eq:history.future.FoI.total;value}{{E.8c}{24}{Existence of the momentum peak}{equation.170}{}}
\newlabel{theory:eq:history.future.FoI.total;value@cref}{{[subequation][3][2147483647,8]E.8c}{[1][24][]24}{}{}{}}
\newlabel{theory:app:timechange}{{F}{24}{Time transformation to map a general epidemic onto the SIR model}{appendix.171}{}}
\newlabel{theory:app:timechange@cref}{{[appendix][6][2147483647]F}{[1][24][]24}{}{}{}}
\newlabel{theory:app:LambertW}{{G}{25}{\texorpdfstring {Lambert's $W$-function}{Lambert's W-function}}{appendix.177}{}}
\newlabel{theory:app:LambertW@cref}{{[appendix][7][2147483647]G}{[1][24][]25}{}{}{}}
\newlabel{theory:eq:Wid}{{G.1}{25}{\texorpdfstring {Lambert's $W$-function}{Lambert's W-function}}{equation.178}{}}
\newlabel{theory:eq:Wid@cref}{{[subequation][1][2147483647,7]G.1}{[1][24][]25}{}{}{}}
\newlabel{theory:app:Rn.from.lamp}{{H}{25}{\texorpdfstring {$\Rn \xm $ from $\lamp $}{R0 x- from lambda+}}{appendix.181}{}}
\newlabel{theory:app:Rn.from.lamp@cref}{{[appendix][8][2147483647]H}{[1][25][]25}{}{}{}}
\newlabel{theory:eq:Rnxp.of.Rnxm}{{H.1}{25}{\texorpdfstring {$\Rn \xm $ from $\lamp $}{R0 x- from lambda+}}{equation.182}{}}
\newlabel{theory:eq:Rnxp.of.Rnxm@cref}{{[equation][1][2147483647,8]H.1}{[1][25][]25}{}{}{}}
\newlabel{theory:eq:Rn.via.Lapp}{{H.2}{25}{\texorpdfstring {$\Rn \xm $ from $\lamp $}{R0 x- from lambda+}}{equation.183}{}}
\newlabel{theory:eq:Rn.via.Lapp@cref}{{[equation][2][2147483647,8]H.2}{[1][25][]25}{}{}{}}
\newlabel{theory:app:zp.min}{{I}{25}{Extrema of prior immunity and final size as a function of \texorpdfstring {$\Rn $}{R0}}{appendix.184}{}}
\newlabel{theory:app:zp.min@cref}{{[appendix][9][2147483647]I}{[1][25][]25}{}{}{}}
\newlabel{theory:eq:Yofx.root.equation}{{I.1}{25}{Extrema of prior immunity and final size as a function of \texorpdfstring {$\Rn $}{R0}}{equation.185}{}}
\newlabel{theory:eq:Yofx.root.equation@cref}{{[equation][1][2147483647,9]I.1}{[1][25][]25}{}{}{}}
\newlabel{theory:eq:dxpm.dxpeak}{{I.2}{25}{Extrema of prior immunity and final size as a function of \texorpdfstring {$\Rn $}{R0}}{equation.186}{}}
\newlabel{theory:eq:dxpm.dxpeak@cref}{{[equation][2][2147483647,9]I.2}{[1][25][]25}{}{}{}}
\newlabel{theory:eq:zpmin.endpoint.immunity.derivative}{{I.3}{25}{Extrema of prior immunity and final size as a function of \texorpdfstring {$\Rn $}{R0}}{equation.187}{}}
\newlabel{theory:eq:zpmin.endpoint.immunity.derivative@cref}{{[equation][3][2147483647,9]I.3}{[1][25][]25}{}{}{}}
\newlabel{theory:eq:zpmin.zp.difference.immunity}{{I.4}{26}{Extrema of prior immunity and final size as a function of \texorpdfstring {$\Rn $}{R0}}{equation.188}{}}
\newlabel{theory:eq:zpmin.zp.difference.immunity@cref}{{[equation][4][2147483647,9]I.4}{[1][26][]26}{}{}{}}
\newlabel{theory:eq:zpmin.zp.derivative.difference}{{I.5}{26}{Extrema of prior immunity and final size as a function of \texorpdfstring {$\Rn $}{R0}}{equation.189}{}}
\newlabel{theory:eq:zpmin.zp.derivative.difference@cref}{{[equation][5][2147483647,9]I.5}{[1][26][]26}{}{}{}}
\newlabel{theory:eq:zpmin.dzp.factorization}{{I.6}{26}{Extrema of prior immunity and final size as a function of \texorpdfstring {$\Rn $}{R0}}{equation.190}{}}
\newlabel{theory:eq:zpmin.dzp.factorization@cref}{{[equation][6][2147483647,9]I.6}{[1][26][]26}{}{}{}}
\newlabel{theory:eq:zpmin.Phi1.Phi2}{{I.7}{26}{Extrema of prior immunity and final size as a function of \texorpdfstring {$\Rn $}{R0}}{equation.191}{}}
\newlabel{theory:eq:zpmin.Phi1.Phi2@cref}{{[equation][7][2147483647,9]I.7}{[1][26][]26}{}{}{}}
\newlabel{theory:eq:zpmin.Phi2.derivative.xpeak}{{I.8}{26}{Extrema of prior immunity and final size as a function of \texorpdfstring {$\Rn $}{R0}}{equation.192}{}}
\newlabel{theory:eq:zpmin.Phi2.derivative.xpeak@cref}{{[equation][8][2147483647,9]I.8}{[1][26][]26}{}{}{}}
\newlabel{theory:eq:zpmin.Phi2.derivative.Rn.stationary}{{I.9}{26}{Extrema of prior immunity and final size as a function of \texorpdfstring {$\Rn $}{R0}}{equation.193}{}}
\newlabel{theory:eq:zpmin.Phi2.derivative.Rn.stationary@cref}{{[equation][9][2147483647,9]I.9}{[1][26][]26}{}{}{}}
\newlabel{theory:eq:zpmin.minimum.condition}{{I.10}{26}{Extrema of prior immunity and final size as a function of \texorpdfstring {$\Rn $}{R0}}{equation.194}{}}
\newlabel{theory:eq:zpmin.minimum.condition@cref}{{[equation][10][2147483647,9]I.10}{[1][26][]26}{}{}{}}
\newlabel{theory:eq:zpmin.log.expansion.near.xinit}{{I.11}{27}{Extrema of prior immunity and final size as a function of \texorpdfstring {$\Rn $}{R0}}{equation.195}{}}
\newlabel{theory:eq:zpmin.log.expansion.near.xinit@cref}{{[equation][11][2147483647,9]I.11}{[1][26][]27}{}{}{}}
\newlabel{theory:eq:zpmin.roots.near.xinit}{{I.12}{27}{Extrema of prior immunity and final size as a function of \texorpdfstring {$\Rn $}{R0}}{equation.196}{}}
\newlabel{theory:eq:zpmin.roots.near.xinit@cref}{{[equation][12][2147483647,9]I.12}{[1][27][]27}{}{}{}}
\newlabel{theory:eq:zpmin.small.upper.bound}{{I.13}{27}{Extrema of prior immunity and final size as a function of \texorpdfstring {$\Rn $}{R0}}{equation.197}{}}
\newlabel{theory:eq:zpmin.small.upper.bound@cref}{{[equation][13][2147483647,9]I.13}{[1][27][]27}{}{}{}}
\newlabel{theory:eq:zpmin.double.root.expansion.point}{{I.14}{27}{Extrema of prior immunity and final size as a function of \texorpdfstring {$\Rn $}{R0}}{equation.198}{}}
\newlabel{theory:eq:zpmin.double.root.expansion.point@cref}{{[equation][14][2147483647,9]I.14}{[1][27][]27}{}{}{}}
\newlabel{theory:eq:zpmin.xpeakstar.expansion}{{I.15}{27}{Extrema of prior immunity and final size as a function of \texorpdfstring {$\Rn $}{R0}}{equation.199}{}}
\newlabel{theory:eq:zpmin.xpeakstar.expansion@cref}{{[equation][15][2147483647,9]I.15}{[1][27][]27}{}{}{}}
\newlabel{theory:app:general.z}{{J}{27}{Generalization of the removed compartment}{appendix.200}{}}
\newlabel{theory:app:general.z@cref}{{[appendix][10][2147483647]J}{[1][27][]27}{}{}{}}
\newlabel{theory:eq:XYF;Z}{{J.1}{27}{Generalization of the removed compartment}{equation.201}{}}
\newlabel{theory:eq:XYF;Z@cref}{{[equation][1][2147483647,10]J.1}{[1][27][]27}{}{}{}}
\newlabel{theory:eq:YZ.incidence.history}{{J.2}{27}{Generalization of the removed compartment}{equation.202}{}}
\newlabel{theory:eq:YZ.incidence.history@cref}{{[equation][2][2147483647,10]J.2}{[1][27][]27}{}{}{}}
\newlabel{theory:eq:re;Z}{{J.3}{27}{Generalization of the removed compartment}{equation.203}{}}
\newlabel{theory:eq:re;Z@cref}{{[equation][3][2147483647,10]J.3}{[1][27][]27}{}{}{}}
\newlabel{theory:app:epimom.Rt}{{K}{28}{Time-varying reproduction number}{appendix.204}{}}
\newlabel{theory:app:epimom.Rt@cref}{{[appendix][11][2147483647]K}{[1][27][]28}{}{}{}}
\newlabel{theory:eq:Rt.def}{{K.1}{28}{Time-varying reproduction number}{equation.205}{}}
\newlabel{theory:eq:Rt.def@cref}{{[equation][1][2147483647,11]K.1}{[1][28][]28}{}{}{}}
\newlabel{theory:eq:Rt.sep}{{K.2}{28}{Time-varying reproduction number}{equation.206}{}}
\newlabel{theory:eq:Rt.sep@cref}{{[equation][2][2147483647,11]K.2}{[1][28][]28}{}{}{}}
\newlabel{theory:eq:re.Rt}{{K.3}{28}{Time-varying reproduction number}{equation.207}{}}
\newlabel{theory:eq:re.Rt@cref}{{[subequation][3][2147483647,11]K.3}{[1][28][]28}{}{}{}}
\newlabel{theory:eq:re.Rt;X}{{K.3a}{28}{Time-varying reproduction number}{equation.208}{}}
\newlabel{theory:eq:re.Rt;X@cref}{{[subequation][1][2147483647,3]K.3a}{[1][28][]28}{}{}{}}
\newlabel{theory:eq:re.Rt;FoI}{{K.3b}{28}{Time-varying reproduction number}{equation.209}{}}
\newlabel{theory:eq:re.Rt;FoI@cref}{{[subequation][2][2147483647,3]K.3b}{[1][28][]28}{}{}{}}
\newlabel{theory:eq:Ra.Rt}{{K.4}{28}{Time-varying reproduction number}{equation.210}{}}
\newlabel{theory:eq:Ra.Rt@cref}{{[equation][4][2147483647,11]K.4}{[1][28][]28}{}{}{}}
\newlabel{theory:eq:re.Y.Rt}{{K.5}{28}{Time-varying reproduction number}{equation.211}{}}
\newlabel{theory:eq:re.Y.Rt@cref}{{[equation][5][2147483647,11]K.5}{[1][28][]28}{}{}{}}
\newlabel{theory:eq:dYdtau.Rt}{{K.6c}{28}{Time-varying reproduction number}{equation.215}{}}
\newlabel{theory:eq:dYdtau.Rt@cref}{{[subequation][3][2147483647,6]K.6c}{[1][28][]28}{}{}{}}
\newlabel{theory:eq:dYdx.Rt}{{K.7}{28}{Time-varying reproduction number}{equation.216}{}}
\newlabel{theory:eq:dYdx.Rt@cref}{{[equation][7][2147483647,11]K.7}{[1][28][]28}{}{}{}}
\makeatother

